A Unified View of Evaluation Metrics for Structured Prediction

We present a conceptual framework that unifies a variety of evaluation metrics for different structured prediction tasks (e.g. event and relation extraction, syntactic and semantic parsing). Our framework requires representing the outputs of these tasks as objects of certain data types, and derives metrics through matching of common substructures, possibly followed by normalization. We demonstrate how commonly used metrics for a number of tasks can be succinctly expressed by this framework, and show that new metrics can be naturally derived in a bottom-up way based on an output structure. We release a library that enables this derivation to create new metrics. Finally, we consider how specific characteristics of tasks motivate metric design decisions, and suggest possible modifications to existing metrics in line with those motivations.

==> appendices/coref.tex <==



\subsection{MUC}
 The widely used MUC metric for coreference resolution \citep{vilain-etal-1995-model} is a link-based metric  that reports precision, recall, and $\rm F_1$ for the links denoting the coreference relationships between mentions.\footnote{~The MUC metric is not to be confused with the metrics presented in \S\ref{subsec:tf} for scoring template filling on MUC-4.}  MUC computes its recall as 
\begin{equation}
    \recall_{\rm MUC} = \frac{\sum_{r\in R} (\left|r\right| - \left|p_P(r)\right|)}{\sum_{r\in R} (\left| r\right| - 1)},
\end{equation}
where $p_P(r)$ is the partition of $r$ with $P$, the predicted set of entities. Note that the nominator can be written as $\sum_{r \in R}\left( \sum_{I \in p_P(r)} \left|I\right| - 1 \right)$: thus we can define the number of shared coreference links as a similarity function between entities:
\begin{equation}
    \phi_{\rm link}(X, Y) = \max\{0, \left| X \cap Y \right| - 1\}.
\end{equation}
Then we have the following using unconstrained matching:
\begin{equation}
    \recall_{\rm MUC} = \recall^{\sim}_\texttt{entities}[\phi_{\rm link}].
\end{equation}
Precision / ${\rm F}_1$ can be defined similarly.


% To lightly adapt an example from \citet{vilain-etal-1995-model}, suppose we have a reference entity $R = \{A, B, C\}$ and suppose its mentions are split in the system output across two predicted entities $P_1 = \{A, C\}$ and $P_2 = \{B, D\}$. For item (2) above, ``constructing'' $R$ by linking $A$, $B$, and $C$ requires two links (any two of $A \leftrightarrow B$, $B \leftrightarrow C$, and $A \leftrightarrow C$). In general, an entity of $|R|$ mentions can be described by $|R| - 1$ links between mentions. For item (1) above, constructing an entity $P$ from $P_1$ and $P_2$ such that $R \subseteq P$ just requires bridging $P_1$ and $P_2$ with one additional link (either $A \leftrightarrow B$ or $B \leftrightarrow C$). Thus, recall is $\frac{1}{2}$. In general, if the system output $\{P_1, \ldots, P_n\}$ partitions the mentions of reference entity $R$ into partition $p(R) = \{P_i \cap R : |P_i \cap R| > 0, i \in \{1, \ldots, n\}\}$, recall for entity $R$ is given by Eq.\ \ref{eq:muc-entity-recall}. \emph{Overall} recall, given in Eq.\ \ref{eq:muc-total-recall}, just sums the numerator and denominator of Eq.\ \ref{eq:muc-entity-recall} over all reference entities:
% \begin{align}
%     \text{recall}(R) &= \frac{(|R| - |p(R)|)}{(|R| - 1)}\label{eq:muc-entity-recall} \\
%     \text{recall}_{\text{total}} &= \frac{\sum_i (|R_i| - |p(R_i)|)}{\sum_i (|R_i| - 1)}\label{eq:muc-total-recall}
% \end{align}
% To compute precision, one simply swaps the roles of the predicted and reference entities in Eqs.\ \ref{eq:muc-entity-recall} and \ref{eq:muc-total-recall}. That is, we compute how many additional links we need between elements of the \emph{reference}-induced partition $p(P) = \{R_i \cap P : |R_j \cap P| > 0, j \in \{1, \ldots, m\}\}$ of \emph{predicted} entity $P$ such that $P \subseteq R$, replacing $R$ with $P$ in the above equations:
% \begin{align}
%     \text{precision}(P) &= \frac{(|P| - |p(P)|)}{(|P| - 1)}\label{eq:muc-entity-precision} \\
%     \text{precision}_{\text{total}} &= \frac{\sum_j (|P_j| - |p(P_j)|)}{\sum_j (|P_j| - 1)}\label{eq:muc-total-precision}
% \end{align}
% To show how MUC fits into our framework, we would like to be able to write Eqs. \ref{eq:muc-total-recall} and \ref{eq:muc-total-precision} as $\recall-$ and $\precision-$normalized sums of similarity functions between pairs of entities. Let us first focus on Eq. \ref{eq:muc-entity-recall}. If we suppose, as \citeauthor{vilain-etal-1995-model} do, that any reference mention that is not explicitly linked to any other mention in the predictions forms a singleton, then we can write our entity similarity function as:
% \begin{equation}
%     \phi_\texttt{Entity}(P,R) =
%     \begin{cases}
%     |P \cap R| - 1, &\text{ if } |P \cap R| > 0 \\
%     0, &\text{otherwise}
%     \end{cases}\label{eqn:muc-score-revised}
% \end{equation}
% For fixed $R$, summing Eq. \ref{eqn:muc-score-revised} over $P$ will yield the numerator of Eq. \ref{eq:muc-entity-recall}: summing $|P \cap R|$ over $P$ yields $|R|$ and summing 1 over all predicted entities $P$ where $|P \cap R| > 0$ just counts the number of predicted entities that partition $R$ (i.e. $|p(R)|$). Similarly, for fixed $P$, summing Eq. \ref{eqn:muc-score-revised} over $R$ will yield the numerator of Eq. \ref{eq:muc-entity-precision}.
 


\subsection{$B^3$}
$B^3$ \citep{bagga1998algorithms} tries to solve two problems with MUC: first, MUC's failure to reward correct identification of singleton entities (since it counts \emph{links} only), and second, its intrinsic bias in favor of system outputs containing fewer entities. However, it has numerous problems of its own \citep{luo-2005-coreference, moosavi-strube-2016-coreference, luo2016evaluation}. For instance, \citet{luo2016evaluation} note that if a given reference mention is repeated across multiple predicted entities, $B^3$ will award credit for each one.

In contrast to MUC, $B^3$ focuses on \emph{mentions}. Suppose $P_m$ and $R_m$ are the predicted and reference entities that contain mention $m$, and suppose $c(P_m)$ is the number of correct mentions in $P_m$, i.e.:
\begin{equation}
c(P_m) = |P_m \cap R_m| = \phi_3(P_m, R_m)
\end{equation}
$B^3$ computes $m$-specific precision and recall as:
\begin{align}
    \text{precision}(m) &= \frac{c(P_m)}{|P_m|}\label{eq:b3-mention-precision} \\
    \text{recall}(m) &= \frac{c(P_m)}{|R_m|}\label{eq:b3-mention-recall}
\end{align}
It then computes overall precision and recall as a weighted average over all mentions $m$:
\begin{align}
    \text{precision}_\text{total} &= \sum_{m \in M} w_m \cdot \text{precision}(m)\label{eq:b3-total-precision} \\
    \text{recall}_\text{total} &= \sum_{m \in M} w_m \cdot \text{recall}(m)\label{eq:b3-total-recall}
\end{align}
where $M$ is the set of all predicted mentions.\footnote{This is the ``informal'' formulation of $B^3$ described in \citet{bagga1998algorithms}. See their paper, as well as \citet{moosavi-strube-2016-coreference} for alternative, equivalent formulations.} \citeauthor{bagga1998algorithms} use a weighted average to allow for heavier weighting of mentions that are ``more important,'' according to whatever notion of importance may be applicable.\footnote{The notion of mention informativity, discussed in \S\ref{sec:discussion}, would be one example.} However, the standard practice is to use the same weight for all $m$.

Although $B^3$ is a mention-level metric, it can nonetheless be viewed as computing a score over an unconstrained alignment ($A^\sim$) between \emph{entities}. The question, then, is what the entity similarity function is. To start, consider that $c(P_m)$ is the same for all mentions $m \in P_m \cap R_m$, as is the denominator of Eqs. \ref{eq:b3-mention-precision} and \ref{eq:b3-mention-recall}. Thus, Eqs. \ref{eq:b3-mention-precision} and \ref{eq:b3-mention-recall} as a whole are equivalent for all mentions $m \in P_m \cap R_m$. This in turn implies that there will be $|P_m \cap R_m|$ copies of $\text{precision}(m)$ in the sum of Eq. \ref{eq:b3-total-precision} and the same number of copies of $\text{recall}(m)$ in the sum of Eq. \ref{eq:b3-total-recall}. The trouble is that, owing to the per-mention normalization in Eqs. \ref{eq:b3-mention-precision} and \ref{eq:b3-mention-recall}, we cannot write Eqs. \ref{eq:b3-total-precision} and \ref{eq:b3-total-recall} as $\precision$- and $\recall$-normalized sums (respectively) of the same similarity function between entity pairs. Rather, we must define different similarities for precision and for recall:
\begin{align}
    \phi_\texttt{Entity-R}(P,R) &= \frac{|P \cap R|}{|R|} \sum_{m \in P \cap R} w_m\label{eqn:b3-entity-r-similarity} \\
    \phi_\texttt{Entity-P}(P,R) &= \frac{|P \cap R|}{|P|} \sum_{m \in P \cap R} w_m\label{eqn:b3-entity-p-similarity}
\end{align}
Eqs. \ref{eq:b3-total-precision} and \ref{eq:b3-total-recall} can then be expressed as sums of Eqs. \ref{eqn:b3-entity-r-similarity} and \ref{eqn:b3-entity-p-similarity}, respectively, over all entity pairs.

% $B^3$ presents essentially the same problem for our framework as MUC: we cannot express Eqs. \ref{eq:b3-total-precision} and \ref{eq:b3-total-recall} in terms of sums of similarity functions between entities.

% \subsection{BLANC}
% Like MUC, the BLANC metric \citep{recasens2011blanc, luo-etal-2014-extension} is link-based. However, it distinguishes itself from MUC in part by also considering \emph{non}-coreference links, which connect all pairs of mentions that are \emph{not} coreferent. Let us denote the sets of all predicted and reference \emph{coreference} links as $C_P$ and $C_R$ and the set of all predicted and reference \emph{non-coreference links} as $N_P$ and $N_R$. BLANC computes separate precision and recall scores \emph{over all links} of each type:
% \begin{align}
%     \text{precision}_C &= \frac{|C_P \cap C_R|}{|C_P|} \\
%     \text{precision}_N &= \frac{|N_P \cap N_R|}{|N_P|} \\
%     \text{recall}_C &= \frac{|C_P \cap C_R|}{|C_R|} \\
%     \text{recall}_N &= \frac{|N_P \cap N_R|}{|N_R|}
% \end{align}
% It then computes an overall precision and recall as the average precision and recall between the two link types:
% \begin{align}
%     \text{precision}_\text{total} &= \frac{\text{precision}_C + \text{precision}_N}{2} \\
%     \text{recall}_\text{total} &= \frac{\text{recall}_C + \text{recall}_N}{2}
% \end{align}
% BLANC trivially fits within our framework if viewed as computing a bipartite matching between sets of \emph{links}, where the implicit link similarity function is identity ($\delta_\texttt{link}$). But it also fits within the framework when viewed as unconstrained ($A^\sim$) entity alignment. To see why, consider that every link that is \emph{not} a coreference link is a \emph{non}-coreference link, and vice-versa. Thus, maximizing $|C_P \cap C_R|$ necessarily maximizes $|N_P \cap N_R|$ and vice-versa. Without loss of generality, let us therefore focus on $|C_P \cap C_R|$. Clearly, we can break this set intersection down by entity pairs. Let $P_i \in P$ (where $P_i \subseteq C_P$) denote predicted entity $i \in \{1, \ldots, n\}$ and $R_j \in R$ (where $R_j \subseteq C_R$) denote reference entity $j \in \{1, \ldots, m\}$. Then the unnormalized entity alignment score is given by:
% \begin{equation}
%     \Sigma^\leftrightarrow(P,R) = |C_p \cap C_R| = \sum_{i,j} |P_i \cap R_j|
% \end{equation}
% where the normalizer is either $\precision$ or $\recall$. This is like $\text{CEAF}_{\phi_3}$, except that the alignment is unconstrained and entities are defined in terms of links rather than mentions. Given this alignment, it is then straightforward to compute $\text{precision}_N$ and $\text{recall}_N$, and then to normalize again according to $\text{precision}_\text{total}$ and $\text{recall}_\text{total}$.

==> appendices/todolist.tex <==
\begin{enumerate}
    \item Why alignment metric can be a unified view of SP? We have to justify this is widely used in evaluating structure prediction tasks. 
    \item The atomic operator should have a positive range. Why?
\end{enumerate}
